LeMo-NADe: Multi-Parameter Neural Architecture Discovery with LLMs

Building efficient neural network architectures can be a time-consuming task requiring extensive expert knowledge. This task becomes particularly challenging for edge devices because one has to consider parameters such as power consumption during inferencing, model size, inferencing speed, and CO2 emissions. In this article, we introduce a novel framework designed to automatically discover new neural network architectures based on user-defined parameters, an expert system, and an LLM trained on a large amount of open-domain knowledge. The introduced framework (LeMo-NADe) is tailored to be used by non-AI experts, does not require a predetermined neural architecture search space, and considers a large set of edge device-specific parameters. We implement and validate this proposed neural architecture discovery framework using CIFAR-10, CIFAR-100, and ImageNet16-120 datasets while using GPT-4 Turbo and Gemini as the LLM component. We observe that the proposed framework can rapidly (within hours) discover intricate neural network models that perform extremely well across a diverse set of application settings defined by the user.

==> Table/GPT/cifa10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Effectiveness of our framework for generating optimal neural network models for CIFAR-10 Dataset while using ChatGPT 4.0 as the LLM/AGI.}
\label{tab:gptCifar10}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\renewcommand{\arraystretch}{1.2}
\scriptsize\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{lcccccccr}
\toprule
\textbf{Setting} & \textbf{\begin{tabular}[c]{@{}c@{}}Validation \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number\\ of \\ Params\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Runtime \\ (Hours)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Energy \\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ CO2 \\ Emission \\ (lbs)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing \\ Frame \\ Per \\ Second\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ Energy \\ Per Image\\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ CO2 \\ Emission \\ (lbs)\end{tabular}} \\ 

\midrule
1                & 84.02 \%                                                                & 2442698                                                                & 3.93                                                                                          & 0.51569                                                                                       & 0.4919689                                                                                           & 6897.222                                                                               & 1.11E-05                                                                                      & 1.06E-05                                                                                \\ 
2                & 85.44 \%                                                                & 357706                                                                 & 4.60                                                                                          & 0.56821                                                                                       & 0.5420745                                                                                           & 115220.68                                                                              & 5.34E-06                                                                                      & 5.09E-06                                                                                \\ 
3                & 90.90 \%                                                                & 699466                                                                 & 4.25                                                                                          & 0.70407                                                                                       & 0.6716806                                                                                           & 10755.78                                                                               & 7.06E-06                                                                                      & 6.74E-06                                                                                \\ 
4                & 70.21 \%                                                                & 136874                                                                 & 4.84                                                                                          & 0.47512                                                                                       & 0.4532650                                                                                           & 14636.72                                                                               & 5.39E-06                                                                                      & 5.14E-06                                                                                \\ 
5                & 86.64 \%                                                                & 2400330                                                                & 4.27                                                                                          & 0.57434                                                                                       & 0.5479185                                                                                           & 13051.73                                                                               & 5.89E-06                                                                                      & 5.62E-06                                                                                \\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> Table/GPT/cifar100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Effectiveness of our framework for generating optimal neural network models for CIFAR-100 Dataset while using ChatGPT 4.0 as the LLM/AGI.}
\label{tab:gptCifar100}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\renewcommand{\arraystretch}{1.2}
\scriptsize\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{lcccccccr}
\toprule
\textbf{Setting} & \textbf{\begin{tabular}[c]{@{}c@{}}Validation \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number\\ of \\ Params\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Runtime \\ (Hours)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Energy \\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ CO2 \\ Emission \\ (lbs)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing \\ Frame \\ Per \\ Second\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ Energy \\ Per Image\\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ CO2 \\ Emission \\ (lbs)\end{tabular}} \\ 

\midrule
1                & 56.20\%                                                                 & 948708                                                                 & 4.46                                                                                          & 0.68742                                                                                       & 0.6557942                                                                                                                & 11753.98                                                                               & 7.95E-06                                                                                      & 7.59E-06                                                                                \\ 
2                & 63.62\%                                                                 & 1725348                                                                & 4.73                                                                                          & 0.71416                                                                                       & 0.6813068                                                                                                                & 10278.36                                                                               & 6.08E-06                                                                                      & 5.80E-06                                                                                \\ 
3                & 58.24\%                                                                 & 948708                                                                 & 4.13                                                                                          & 0.60556                                                                                       & 0.5777015                                                                                                                & 13294.64                                                                               & 5.96E-06                                                                                      & 5.68E-06                                                                                \\ 
4                & 68.38\%                                                                 & 79530                                                                  & 4.81                                                                                          & 0.50212                                                                                       & 0.4790213                                                                                                                & 15079.86                                                                               & 5.63E-06                                                                                      & 5.37E-06                                                                                \\
5                & 63.90\%                                                                 & 3489316                                                                & 4.68                                                                                          & 0.73515                                                                                       & 0.7013343                                                                                                                & 10026.15                                                                               & 7.44E-06                                                                                      & 7.10E-06                                                                                \\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> Table/Gemini/cifar10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Effectiveness of our framework for generating optimal neural network models for CIFAR-10 Dataset while using Gemini as the LLM/AGI.}
\label{tab:geminiCifar10}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\renewcommand{\arraystretch}{1.2}
\scriptsize\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{lcccccccr}
\toprule
\textbf{Setting} & \textbf{\begin{tabular}[c]{@{}c@{}}Validation \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number\\ of \\ Params\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Runtime \\ (Hours)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Energy \\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ CO2 \\ Emission \\ (lbs)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing \\ Frame \\ Per \\ Second\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ Energy \\ Per Image\\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ CO2 \\ Emission \\ (lbs)\end{tabular}} \\ 

\midrule
1                & 82.94 \%                                                                & 440778                                                                & 2.14                                                                                         & 0.16051                                                                                     & 0.1531                                                                                          & 13435.93                                                                              & 3.18e-06                                                                                     & 3.04e-06                                                                               \\ 
2                & 81.52 \%                                                                & 128842                                                                 & 2.79                                                                                        & 0.2333                                                                                      & 0.2226                                                                                           & 21553.23                                                                    & 2.44e-06                                                                                      & 2.33e-06                                                                                \\ 
3                & 82.14 \%                                                                & 3016522                                                                 & 2.403                                                                                         & 0.20635                                                                                  & 0.19686                                                                                          & 20460.87                                                                            & 1.08e-06                                                                                      &1.03e-06                                                                                \\ 
4                & 71.68 \%                                                                & 79530                                                                 & 2.83                                                                                       & 0.1786                                                                                       & 0.1704                                                                                           & 23029.86                                                                               & 7.42e-07                                                                                      & 7.08e-07                                                                               \\ 
5                & 79.48 \%                                                                & 1276234                                                                & 1.94                                                                                        & 0.12644                                                                                       & 0.1206                                                                                           & 19565.53                                                                             & 6.42E-06                                                                                      &6.12E-06                                                                                \\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> Table/Gemini/cifar100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{Effectiveness of our framework for generating optimal neural network models for CIFAR-100 Dataset while using Gemini as the LLM/AGI.}
\label{tab:geminiCifar10}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\renewcommand{\arraystretch}{1.2}
\scriptsize\addtolength{\tabcolsep}{-1pt}
\begin{tabular}{lcccccccr}
\toprule
\textbf{Setting} & \textbf{\begin{tabular}[c]{@{}c@{}}Validation \\ Accuracy\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number\\ of \\ Params\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Runtime \\ (Hours)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ Energy \\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Generating \\ + \\ Training\\ CO2 \\ Emission \\ (lbs)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing \\ Frame \\ Per \\ Second\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ Energy \\ Per Image\\ (kWh-PUE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Inferencing\\ CO2 \\ Emission \\ (lbs)\end{tabular}} \\ 

\midrule
1                & 46.22 \%                                                                & 721060                                                                & 2.21                                                                                        & 0.16087                                                                                       & 0.1535                                                                                           & 21455.82                                                                             & 2.91e-06                                                                                  & 2.77e-06                                                                                \\ 
2                & 52.12 \%                                                                & 801444                                                                 & 2.48                                                                                         & 0.09318                                                                                       & 0.0889                                                                                           & 20740.8                                                                              & 2.48E-06                                                                                      & 2.36E-06                                                                                \\ 
3                & 51.08 \%                                                                & 4385540                                                                 & 2.65                                                                                         & 0.28765                                                                                       & 0.2744                                                                                           & 18524.72                                                                              & 2.67E-06                                                                                      & 2.55E-06                                                                                \\ 
4                & 10.52 \%                                                                & 12836                                                                 & 2.83                                                                                         & 0.10146                                                                                       & 0.0968                                                                                           & 20726.49                                                                              & 1.19E-06                                                                                      & 2.09E-06                                                                                \\ 
5                & 50.80 \%                                                                & 2665124                                                                & 2.92                                                                                          & 0.21153                                                                                       & 0.2018                                                                                           & 18470.16                                                                               & 1.04E-06                                                                                      & 9.90E-07                                                                                \\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
